THOR: A Generic Energy Estimation Approach for On-Device Training

Battery-powered mobile devices (e.g., smartphones, AR/VR glasses, and various IoT devices) are increasingly being used for AI training due to their growing computational power and easy access to valuable, diverse, and real-time data. On-device training is highly energy-intensive, making accurate energy consumption estimation crucial for effective job scheduling and sustainable AI. However, the heterogeneity of devices and the complexity of models challenge the accuracy and generalizability of existing estimation methods. This paper proposes THOR, a generic approach for energy consumption estimation in deep neural network (DNN) training. First, we examine the layer-wise energy additivity property of DNNs and strategically partition the entire model into layers for fine-grained energy consumption profiling. Then, we fit Gaussian Process (GP) models to learn from layer-wise energy consumption measurements and estimate a DNN's overall energy consumption based on its layer-wise energy additivity property. We conduct extensive experiments with various types of models across different real-world platforms. The results demonstrate that THOR has effectively reduced the Mean Absolute Percentage Error (MAPE) by up to 30%. Moreover, THOR is applied in guiding energy-aware pruning, successfully reducing energy consumption by 50%, thereby further demonstrating its generality and potential.

==> sections/abstract.tex <==
\begin{abstract}
% With a series of breakthrough achievements in the field of \ML and the advancement of hardware devices, \DNN models have been increasingly deployed on a wide range of mobile devices. 
% The deployment of \DNN models on mobile devices is receiving widespread attention. 
% With the 
% Deep Neural Networks (DNN) models are widely deployed to mobile devices to enable on-device \AI training, which provides privacy preserving and real-update updates compared to traditional centralized \AI training on servers.    

Battery-powered mobile devices (e.g., smartphones, tablets, laptops, AR/VR glasses/helmets, and various IoT devices) are taking more \AI training due to their integral roles in daily life, which provides a rich source of highly valuable, diverse, and real-time data. 
However, on-device training is an exceptionally energy-intensive task. 
As a result, it is crucial to accurately estimate energy consumption on mobile devices to facilitate effective job scheduling. 
Nevertheless, due to the heterogeneity of devices and the complexity of models, existing methods based on \FLOPs have not achieved satisfactory accuracy in predictions. 

This paper proposes \sys, a generic method for energy consumption estimation in \DNN training. 
First, we strategically partition the whole model into multiple layers. 
Subsequently, \GP models are fitted based on the consumption observations of the layers.
For estimation, the overall energy consumption of the whole model is obtained by summing the individual energy consumption of each layer. 
We conduct extensive experiments with various types of models across different platforms. 
The results demonstrate that \sys has effectively reduced the \MAPE by up to 30\%. 
Moreover, \sys can illustrate the energy pattern of each layer, which paves the way for more efficient on-device training and job scheduling. 
\end{abstract}

% motivation: Layer wise 能耗能拼接

